Sparse Systolic Tensor Array for Efficient CNN Hardware Acceleration

Convolutional neural network (CNN) inference on mobile devices demands efficient hardware acceleration of low-precision (INT8) general matrix multiplication (GEMM). Exploiting data sparsity is a common approach to further accelerate GEMM for CNN inference, and in particular, structural sparsity has the advantages of predictable load balancing and very low index overhead. In this paper, we address a key architectural challenge with structural sparsity: how to provide support for a range of sparsity levels while maintaining high utilization of the hardware. We describe a time unrolled formulation of variable density-bound block (VDBB) sparsity that allows for a configurable number of non-zero elements per block, at constant utilization. We then describe a systolic array microarchitecture that implements this scheme, with two data reuse optimizations. Firstly, we increase reuse in both operands and partial products by increasing the number of MACs per PE. Secondly, we introduce a novel approach of moving the IM2COL transform into the hardware, which allows us to achieve a 3x data bandwidth expansion just before the operands are consumed by the datapath, reducing the SRAM power consumption. The optimizations for weight sparsity, activation sparsity and data reuse are all interrelated and therefore the optimal combination is not obvious. Therefore, we perform an design space evaluation to find the pareto-optimal design characteristics. The resulting design achieves 16.8 TOPS/W in 16nm with modest 50% model sparsity and scales with model sparsity up to 55.7TOPS/W at 87.5%. As well as successfully demonstrating the variable DBB technique, this result significantly outperforms previously reported sparse CNN accelerators.

==> rebuttal.tex <==
We've revised the paper significantly based on reviewer feedback, and added a new extensive comparison in Table 7.


Reviewer-A

Q-A1: How do you convert a matrix to DBB format?
A-A1: It's necessary to train the model with DBB constraints (Section 5.1).

Q-A2: How do you find the sweet spot of NNZ?
A-A2: We've added a brief sensitivity analysis of block-size/NNZ in Table 4 (Section 6.6).

Q-A3: Does the baseline keep the same performance (throughput)?
A-A3: Yes, the performance/throughput is the same as the baseline in all cases, indicated in figure captions as "iso-throughput".

Q-A4: It would be clearer to show the area/power as a percentage of the baseline.
A-A4: Done.


Reviewer-B

Q-B1: Lack of CNN performance in evaluation.
A-B1: All results are "iso-throughput": designs achieve equal throughput to the baseline. Energy/area reduction is then quoted compared to the baseline at the equal throughput.

Q-B2: Comparison with: (Wei-NeurIPS-2016), (Zhou-MICRO-2018), (Deng-MICRO-2018). 
A-B2: [Deng-MICRO-2018]-[19] only targets FC/dense layers, so not directly comparable (mentioned in related work).  [Wei-Neurips-2016]-[51], discussed in Section 2.2 - algorithm only, not an accelerator paper.  [Zhou-MICRO-2018]-[55] is now shown in new Table 7, Section 7.2.  SiSTA results are much better due to efficient microarchitecture.

Q-B3: Inference performance vs CPU/GPU/random sparse accelerator/other structured-sparse accelerators?
A-B3: CPU/GPU cannot benefit from DBB without custom instructions. It is well known that CPU/GPU have significantly worse performance than accelerators, e.g. Nvidia TU100 GPU achieves ~0.86TOPS/W, so we don't bother to compare.  A broad comparison with state-of-the-art accelerators is given in new Table 7.

Q-B4: In section 6.1, the authors choose only one baseline with a different network model. They should evaluate on the same CNN models comparing accuracy, sparse ratio.
A-B4: The only goal of Section 6.1 is simply to demonstrate that DBB training has a negligible impact on accuracy.  An extensive evaluation of sparse models is beyond the scope of this work, which focuses on NPU microarchitecture.

Q-B5: In Table 2, structured-sparse accelerators should be added as baseline.
A-B5: We've added direct comparison with Cambricon-S and Kang et al. in new Table 7.

Q-B6: Throughput or latency of STA-DBB is missing.
A-B6: All results given are at "iso-throughput" to the baseline, as noted in the figure captions.  


Reviewer-C

Q-C1: How is DBB different from: (i) Kang-TCSVT'2019, (ii) Zhang-HotChips'2019.
A-C1: Ref (i)[26] uses the same sparsity constraint, but implements dot-product datapaths, with low reuse compared to our NPU.  Direct comparison is given in new Table 7.
Ref (ii)[50] is sparse matrix-vector, not CNN, and is an oral presentation rather than a paper; added to background.

Q-C2: Missing discussion of depthwise-separable layers.
A-C2: We apply DBB to the pointwise layers only, which anyway constitute the majority of the operations. For the 3x3s, we fall back to supporting dense operation, which is a key feature of this work.  We've clarified this in Section 6.1.  

Q-C3: Novelty is limited to a vector core in systolic array, IM2Col, and evaluation across parameters. These account only for incremental novelty.
A-C3: We think our work demonstrates that microarchitecture is critical in NPU design.  Overall, our contributions of 1) STA, 2) STA-DBB, 3) hardware IM2COL, and 4) design space exploration for balanced reuse, result in significantly higher energy and area efficiency than previous work - 8.75x better TOPS/W than the previous state-of-the-art (Laconic): 5.5x for STA only, 7.0x for STA-DBB and 8.75x for STA-DBB-IM2COL. We think this will be of great interest to Micro attendees.


Reviewer-D

Q-D1: How is IOFMB accessed by the MCU? Is the data layout friendly for both TPE and MCU?
A-D1: The IOFMB/WB SRAMs are internally memory-mapped to the MCU, for DMA and data processing tasks.  The data layout is optimized for the TPE array, with the activations organized as compact INT8 HxWxC tensors, later expanded by the inline HW IM2COL. IOFMB is also double buffered between array and MCU to relax timing.

Q-D2 Provide details on how the architecture (area/power/performance) comparison with Laconic, and/or SMT-SA (for INT8) is justified.
A-D2: Added Table 7 for broad comparison with prior work.


Reviewer-E

Q-E1: Introduction writing can be improved.
A-E1: Improved in revision.

Q-E2: Sista appears to handle any type of layers, not only CNN?
A-E2: Yes, this work is essentially a heavily optimized GEMM hardware accelerator.  We have updated the title slightly to reflect this sentiment.

Q-E3: Fig4(b) and Fig5: Shouldn’t there be one accumulator next to each DPE?
A-E3: TPE has two types of registers: 1) accumulators inside the MAC, and 2) operand pipeline registers.  In Fig. 5, only shows the operand pipeline registers, the accumulators are inside the DP2 blocks.

Q-E4: Sensitivity analysis to block-size/NNZ.
A-E4: Added in Table 4.

Q-E5: Fig9: Why does the best design get smaller from 2-4-16 TOPS?
A-E5: The normalized area shrinks from 2-8-16 TOPS as the SRAM size is fixed to 1MB and the datapath occupies more increasing proportion of area.

